Cautious Planning with Incremental Symbolic Perception: Designing Verified Reactive Driving Maneuvers

This work presents a step towards utilizing incrementally-improving symbolic perception knowledge of the robot's surroundings for provably correct reactive control synthesis applied to an autonomous driving problem. Combining abstract models of motion control and information gathering, we show that assume-guarantee specifications (a subclass of Linear Temporal Logic) can be used to define and resolve traffic rules for cautious planning. We propose a novel representation called symbolic refinement tree for perception that captures the incremental knowledge about the environment and embodies the relationships between various symbolic perception inputs. The incremental knowledge is leveraged for synthesizing verified reactive plans for the robot. The case studies demonstrate the efficacy of the proposed approach in synthesizing control inputs even in case of partially occluded environments.

==> IROS/Perception.tex <==
%!TEX root = main.tex
\newcommand{\emptys}{\tikz{\node[rectangle, draw,inner sep=6pt] {};}}
\newcommand{\obj}{\tikz{\node[rectangle, draw,inner sep=6pt, fill=black] {};}} \newcommand{\warn}{\includegraphics[width=0.5cm]{DE/warning/empty_warning}} \newcommand{\minor}{\includegraphics[width=0.5cm]{DE/warning/crossroads_with_a_minor_road}} \newcommand{\tsign}{\includegraphics[width=0.5cm]{DE/warning/traffic_signals_ahead}}
\newcommand{\yield}{\includegraphics[width=0.5cm]{DE/priority/yield}}
\newcommand{\bsign}{\includegraphics[width=0.5cm]{DE/special_regulations/Blue}}
\newcommand{\peds}{\includegraphics[width=0.5cm]{DE/special_regulations/pedestrian_crossing}}
\newcommand{\pedz}{\includegraphics[width=0.5cm]{DE/special_regulations/pedestrian_zone}}


We build a  model of the  perception based on 7 variables $o_i$ with $i=1,2,3,\ldots, 7$ that represent the identified objects in the seven grids in Figure \ref{fig:roadcasestudy}. 

As a first instance, consider modelling the lights at intersections. We consider two levels of knowledge. At the first level, for intersections father away the car can only know whether there is an intersection with a light or not. At the second level, it also knows what the color of the light is. 










Variables can take on  $\{$\tikz{\node[rectangle, draw,inner sep=6pt] {};}, 
\tikz{\node[rectangle, draw,inner sep=6pt, fill=black] {};} \includegraphics[width=0.5cm]{DE/warning/empty_warning}, \includegraphics[width=0.5cm]{DE/warning/crossroads_with_a_minor_road}, \includegraphics[width=0.5cm]{DE/warning/traffic_signals_ahead}, 
 \includegraphics[width=0.5cm]{DE/priority/yield}, %
 \includegraphics[width=0.5cm]{DE/special_regulations/Blue}, %
 \includegraphics[width=0.5cm]{DE/special_regulations/pedestrian_crossing}, %
 \includegraphics[width=0.5cm]{DE/special_regulations/pedestrian_zone} $\}$. 
 
 We then have that 
 $o_7, o_6\in  \{$\tikz{\node[rectangle, draw,inner sep=6pt] {};}, 
 \tikz{\node[rectangle, draw,inner sep=6pt, fill=black] {};}$\}$, 
  $o_4, o_5\in  \{$\includegraphics[width=0.5cm]{DE/warning/empty_warning},
 \includegraphics[width=0.5cm]{DE/special_regulations/Blue}$\}$, and 
 $o_{3},o_2,o_1\in \{$  \includegraphics[width=0.5cm]{DE/warning/crossroads_with_a_minor_road}, \includegraphics[width=0.5cm]{DE/warning/traffic_signals_ahead}, 
 \includegraphics[width=0.5cm]{DE/priority/yield}, % 
 \includegraphics[width=0.5cm]{DE/special_regulations/pedestrian_crossing}, %
 \includegraphics[width=0.5cm]{DE/special_regulations/pedestrian_zone}  $\}$. 
 
 Furthermore at each time instance the variables can change based on the perception. We assume that 
 if 
 \begin{align}
 	&(o_i = \emptys)\rightarrow \bigcirc(o_{i-1}=\emptys)\\
 	 	&(o_7 = \obj)\rightarrow \bigcirc(o_{6}=\obj)\\
 	 	&(o_6 = \obj)\rightarrow \bigcirc(o_{5}=\bsign\vee o_{5}=\warn)\\
 	 		& (o_{5}=\bsign )\rightarrow \bigcirc  (o_{4}=\bsign )\\
 & ( o_{5}=\warn)\rightarrow \bigcirc  (  o_{4}=\warn)\\
 & ( o_{4}=\warn)\rightarrow \bigcirc  (o_{3}=\minor\vee o_{3}=\tsign\vee o_{3}=\yield)\\
  & ( o_{4}=\bsign)\rightarrow \bigcirc  (o_{3}=\peds\vee o_{3}=\pedz ) 
  \end{align}
 
 

 

==> IROS/Review.tex <==


\section{Reviewer 1}
Reviewer 3 of IROS 2022 submission 1932

Comments to the author
======================

This paper studied the problem of designing high-level
reactive control of autonomous cars given some symbolic
perception inputs. The authors use abstractions of the
perception module to help with safe control synthesis. One
important contribution is that the proposed hierarchy
enables controller synthesis even in the presence of
uncertainty in observations. In my opinion, this is an
interesting and practical direction, especially in the
field of autonomous driving, and there are many promising
and interesting future directions. The drawback of this
paper is the lack of comparison with existing approaches in
dealing with symbolic inputs, and the lack of real-world
experiments. Besides, I am not sure about the novelty of
using LTL with symbolic inputs for safe control synthesis,
since there were several works about temporal logic
planning with semantic information (e.g: "Optimal temporal
logic planning in probabilistic semantic maps"). For me,
symbolic input is a special category of semantic
information. 


I have the following questions/suggestions/comments for the
authors. 

1). This is a general question. For safe controller
synthesis, one should not only consider the symbolic
perception inputs, but also lots of other environmental
information (e.g. distance information to the obstacle). Do
the authors have any idea or comment about incorporating
other information together with the proposed approach?

2). For the related work section, the authors may consider
adding some existing works that deal with the symbolic
perception inputs, and discuss the advantages of the
proposed approach. 

3). In case study 2, the authors compare the proposed
approach with some conventional approaches. I suggest that
the authors can add a few references there if possible.
Besides, Fig. 5 is not very illustrative to me. The authors
may consider explaining what are the settings for getting
Fig. 5 (e.g. how the frequency of system variables
computed?). 

4). After addressing some other questions mentioned in the
manuscript (e.g. collision avoidance, safe interactions
with pedestrians), I look forward to seeing the authors
deploying the formulations to real robots. 



\medskip 
\section{Reviewer 2} 


Reviewer 5 of IROS 2022 submission 1932

Comments to the author
======================

This paper proposed a method of perception and planning in
autonomous cars. The proposed method is based on
linear-time temporal logic (LTL). Using a multi-resolution
perception model for the environmental state, the planner
can make decisions that reduce the risk under uncertainty
in perception. The issue addressed in this study is
important, and the use of the multi-resolution perception
seems effective. However, there are some concerns listed
below.

There is a concern that some essential references are
missing. This paper mentioned only a few studies that
addressed uncertainty. However, uncertainty in perception
is one of the main challenges in autonomous robots (e.g.,
navigation robots). The authors must refer to some
representative works and describe the difference. For
example, the following studies would relate to this study:
S. Brechtel et al., 2014. (DOI: 10.1109/ITSC.2014.6957722);
C. Hubmann et al., 2018. (DOI: 10.1109/TIV.2017.2788208);
A. Saffiotti, 1997. (DOI: 10.1007/s005000050020)

It may be hard for readers unfamiliar with LTL to
understand the overview of the method. Many symbols were
introduced to precisely formulate the problem and method,
whereas explanations about the overview and intuitive
meaning were few. It is preferred to describe the overview
of the entire method to make it easier to follow. It is
also preferred to explain Equation (2) in the natural
language.

There are also concerns in the evaluation. Why was the
system without multi-resolution perception unable to find
the traffic light? In the setup illustrated in Figure 6, it
would be easier than finding the partially hidden traffic
sign. It is preferred to describe the detail of the Markov
chain model for perception, such as the probability of
perception. It is also desirable to discuss the potential
for the proposed method to be overly conservative. Although
safety is the priority in autonomous cars, being overly
conservative would undermine its usefulness. Discussing
whether this trade-off can be reconciled is beneficial for
readers.

There are other comments listed below:

1) There are symbols that are undefined or defined far
later. For example, there was no definition of the operator
U in Equation 1. Also, the Delta symbol in Definition 1 was
explained in Definition 4; it should be explained in
Definition 1. The meaning of the arrow in Equation (2) was
not described.
2) Figure 6 was referred to before Figure 5.; figures
should be generally numbered in the order in which they are
referenced in the text.
3) The references should also be numbered in the order they
appeared in the text.

==> IROS/intro.tex <==


Autonomous robots can cause serious damage when malfunctioning. Autonomous cars that lead to fatal consequences are the exemplar of the importance of safe autonomy.  Thus, having an autonomous system
that not only adapts to the changing environment but
also guarantees safe behavior becomes crucial. The
problem of high-level reactive control for autonomous
cars is implemented on two modules. The first module, the perception module, measures
the current state of the environment at each step. The second module for motion planning designs and implements
a control plan %towards satisfaction of the endgoal
that takes into account the current environment
state and the current safety and task rules. When operating in a complex environment, these
systems often have involved rules for safety and task
satisfaction.
It has been shown that the design and verification this motion planning module can be automated \cite{fainekos_temporal_2005,finucane_ltlmop_2010}, \cite{kress-gazit_wheres_2007,sahin_multirobot_2019,wang_hyperproperties_2020} 
by using Temporal Logic to express the
safety and functionality properties with logical and temporal
modalities. %, the design and verification of motion planning can be automated \cite{fainekos_temporal_2005,finucane_ltlmop_2010}, \cite{kress-gazit_wheres_2007,sahin_multirobot_2019,wang_hyperproperties_2020}.

\begin{figure}[htp]
	\centering
	\includegraphics[width=.95\columnwidth, trim= .5cm .5cm 1cm 0cm, clip]{IROS/images/motivation.png}
% 	\vspace{-30pt}
	\caption{\small{A motivating example for leveraging partial knowledge about the environment for controlling the ego car. As the car does not have full view of the pedestrian sign, it may still slow down after recognizing the possibility of a warning sign and may have improved chances of reacting in time.}}
 	\label{fig:motivation}
	\vspace{-10pt}
\end{figure}
\indent Consider a very simple case of an autonomous car going down the hill towards a pedestrian crossing as shown in Fig. \ref{fig:motivation}. The yellow translucent rectangle represents the sensing range of the car. This range is limited due to {\color{black} hardware limitations.}
While driving down the slope the car will know there is possibly a warning sign a couple of instances before it actually observes which sign it is.  It is clear that one should take into account all the available information about the perception module, to obtain a verified motion planning module that is neither conservative nor taking unnecessary risk. However,  approaches limited to the motion planning module  \cite{fainekos_temporal_2005,finucane_ltlmop_2010}, \cite{kress-gazit_wheres_2007,sahin_multirobot_2019,wang_hyperproperties_2020}  do not consider the relationship that may exist in the evolution of the current environment state and its uncertainty.

Looking at the presented case, we note that 
if the control module only acts based on exact knowledge of upcoming environment states, the car may have to travel further ahead until the sign fully comes into its sight. This may either force the car to drive very conservatively or it may not leave enough time for the car to slow down to correctly take the pedestrian sign.

% \color{red}
Therefore, in this work we want to encompass 
% However, if we consider 
the interactions between the perception and control modules based on the incremental knowledge about the environment. In this way, we expect that the car may decide to slow down right after detecting a yellow board that there is possibly a ``warning sign" and may later on slow down further after detecting the sign completely.  %This underpins the need for considering multi-level interactions between perception and reactive control modules for the systems which may allow systems to react safely with the environment even when there is some degree of uncertainty associated with the learned parameters. 

\smallskip
In this work, we propose a framework for high-level reactive control design given a symbolic perception input. Abstracting the way of collecting information about the environment state, we instead focus on leveraging the partial knowledge about these variables. The hierarchical relationships between learned variables aid in the decision making process for the ego car.
% \color{black}

To achieve the verifiable usage of perception in motion planning and control as is present in autonomous driving, we will use abstractions to encapsulate the detection and estimation techniques. 
The methods discussed in this work focus on the applications related to autonomous driving in urban setting with limited prior information about the environment. However, the proposed approach can be used in other settings wherein partial knowledge about the environment may lead to a safer control strategy. e.g., search-and-rescue tasks with priority. 


% \noindent{\bfseries Approach.}
% {\disha In this paper, we introduce a hierarchical perception framework for correct-by-construction reactive control synthesis.} To achieve the verifiable usage of machine learning in motion planning and control as is present in autonomous driving, we will use abstractions to encapsulate the learning algorithms. Furthermore, we will abstract the autonomous car into a finite model whose state action updates result both in atomic proposition, but we preserve the information captured by the cars behavior in the abstraction.  We show that this leads to an autonomous car that anticipates changes in traffic signs by slowing down and that actively checks the road condition while driving closer to a  light that can turn red at any moment. 
 %
%
% More precisely, combining the abstract model of the machine learning algorithm and of the motion control and information gathering, we show that assume-guarantee specifications can be used to define and resolve traffic rules for cautious planning with perception and learning algorithms.
%
%% need for 
The main contributions of this work are as follows: 1. We propose a framework for safe high-level reactive control with perception for an autonomous car. 2. We abstract the perception module and establish a hierarchy between these environment variables which facilitates the timely execution of necessary behavior that the system must perform in order to satisfy rules of the road. 3. Additionally, we demonstrate with the help of case studies that this hierarchy helps synthesizing control inputs even in case of partial information about the environment. 

% We establish the inter-relation between the perception and control abstractions. 

% {\disha Contributions: 1. The idea of establishing relations between various learned variables to make high-level decisions with safety guarantees.\\ 
% 2. The inter-relation between evolution of the perception and control abstraction - The knowledge about the current state of the environment determines the behavior of the system which in the next step updates the knowledge about the environment and so on. \\ 
% 3. We abstract the way of gathering information about the environment. Furthermore, we establish hierarchy between various environment variables and model it as a TS. We demonstrate using case studies that this hierarchy allows the system to safely react in time to the events in the environment. \\ 
% 4. We can deal with partial information. \\ 

% }




% \indent Furthermore, a subset of linear temporal logic (LTL), assume-guarantee specifications \cite{bloem2012synthesis} (GR(1)) reduce the otherwise computationally intensive verification and design problem {\disha (exponential-time)} to a polynomial-time design problem. 

{\color{black} The remainder of this paper is structured as follows: Section \ref{sec:literature} reviews the existing approaches addressing the problem at hand. The preliminaries are discussed in Section \ref{sec:prelims} followed by the formal problem definition in Section \ref{sec:Problem}. Section \ref{sec:solution} presents a detailed solution to reactive synthesis and the necessary metric following which Section \ref{sec:case study} presents case studies for different environment conditions.  Section \ref{sec:conclusions} concludes the paper.  
}

\section{Related work}\label{sec:literature}
\indent With respect to the perception module of autonomous systems, numerous approaches have been proposed to improve the perception capabilities %of autonomous systems 
\cite{fayyad2020deep},~\cite{fridman2017autonomous}, \cite{tseng2018combination}. Although the advent of data-driven approaches have greatly improved the perception abilities of autonomous cars, e.g.,~\cite{fridman2017autonomous}, the problems combining perception and decision-making are often dealt with in a sequential way. That is the end-result obtained from the perception module is used as an input to the control synthesis module \cite{okumura2016challenges}. 



Assume guarantee specifications
have been used to obtain a verified reactive control plan for mobile robots in abstract dynamic environments \cite{kress2009temporal}. In \cite{kress2009temporal}, the authors propose a correct-by-construction hybrid reactive controller for bridging up the gap between low and high-level controllers.
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[scale=0.35, trim= 5cm 0cm 0cm 0cm]{IROS/images/motivation.png}
% % 	\vspace{-30pt}
% 	\caption{\small{A motivating example for leveraging partial knowledge about the environment for controlling the ego car. As the car does not have full view of the pedestrian sign, it may still slow down after recognizing the possibility of a warning sign and may have improved chances of reacting in time.}}
%  	\label{fig:motivation}
% 	\vspace{-15pt}
% \end{figure} 
% \indent Towards this end,
Within a similar context,
\cite{kress2011mitigating} addresses the reactivity at specification and control level by using finite abstractions of the system and the environment. They solve a game between sensor propositions that represent the environment and robot propositions to synthesize a reactive control input.   However, both of these works assume an accurate perception input; As opposed to their approach for perception abstraction, in this work we instead consider a perception module in which the information about the environment is incrementally improved. % the  abstraction of perception as a transition system whose transitions depend on the transitions in the control module. 
% {\color{red}[TODO: Double check]}. % checked it (sofie). 
 Using Probabilistic Signal Temporal Logic specifications
\cite{da2021active} proposes a counter-example-guided control synthesis, under perception uncertainty. In contrast to our approach, this approach requires accurate belief models of the perception that quantify the uncertainty of the perception system explicitly.  


% \indent With respect to the perception module of autonomous systems, numerous approaches have been proposed to improve the perception capabilities %of autonomous systems 
% ~\cite{fayyad2020deep},~\cite{fridman2017autonomous}, \cite{tseng2018combination}. Although the advent of data-driven approaches have greatly improved the perception abilities of autonomous cars, e.g.,~\cite{fridman2017autonomous}, the problems combining perception and decision-making are often dealt with in a sequential way. That is the end-result obtained from the perception module is used as an input to the control synthesis module \cite{okumura2016challenges}. 



% \indent These approaches do not consider the relationship that may exist in the learned symbols or parameters. For instance, consider an autonomous car going down the hill towards a pedestrian crossing as shown in Fig. \ref{TODO}. The blue rectangle represents the sensory range of the car. If the system waits for an exact output from the perception module, the car may have to travel further ahead until the sign fully comes into its sight. This may not leave enough time for the car to slow down to correctly take the pedestrian sign. However, if we consider the interactions between the perception and control modules based on the {\color{red} incremental ?} knowledge about the environment, the car may decide to slow down right after detecting a yellow board that there is possibly a ``warning sign" and may later on slow down further after detecting the sign completely. This underpins the need for considering multi-level interactions between perception and reactive control modules for the systems which may allow systems to react safely with the environment even when there is some degree of uncertainty associated with the learned parameters. 

% In this work, we propose a framework for high-level reactive control design given a symbolic perception input. Abstracting the way of collecting information about the environment state, we instead focus on leveraging the partial knowledge about these variables. The hierarchical relationships between learned variables aid in the decision making process for the ego car. The methods discussed in this work focus on the applications related to autonomous driving in urban environments. However, the proposed approach can be used in other settings wherein partial knowledge about the environment may lead to a safer control strategy. e.g., search-and-rescue tasks with priority. To achieve the verifiable usage of perception in motion planning and control as is present in autonomous driving, we will use abstractions to encapsulate the detection and estimation techniques. More precisely, combining the abstract models motion control and information gathering, we show that assume-guarantee specifications can be used to define and resolve traffic rules for cautious planning with perception.  
% % \noindent{\bfseries Approach.}
% % {\disha In this paper, we introduce a hierarchical perception framework for correct-by-construction reactive control synthesis.} To achieve the verifiable usage of machine learning in motion planning and control as is present in autonomous driving, we will use abstractions to encapsulate the learning algorithms. Furthermore, we will abstract the autonomous car into a finite model whose state action updates result both in atomic proposition, but we preserve the information captured by the cars behavior in the abstraction.  We show that this leads to an autonomous car that anticipates changes in traffic signs by slowing down and that actively checks the road condition while driving closer to a  light that can turn red at any moment. 
%  %
% %
% % More precisely, combining the abstract model of the machine learning algorithm and of the motion control and information gathering, we show that assume-guarantee specifications can be used to define and resolve traffic rules for cautious planning with perception and learning algorithms.
% %
% %% need for 
% The main contributions of this work are as follows: 1. We propose a framework for safe high-level reactive control with perception for an autonomous car. 2. We abstract the perception module and establish a hierarchy between these environment variables which facilitates the timely execution of necessary behavior that the system must perform in order to satisfy rules of the road. 3. Additionally, we demonstrate with the help of case studies that this hierarchy helps synthesizing control inputs even in case of partial information about the environment. 

% % We establish the inter-relation between the perception and control abstractions. 

% % {\disha Contributions: 1. The idea of establishing relations between various learned variables to make high-level decisions with safety guarantees.\\ 
% % 2. The inter-relation between evolution of the perception and control abstraction - The knowledge about the current state of the environment determines the behavior of the system which in the next step updates the knowledge about the environment and so on. \\ 
% % 3. We abstract the way of gathering information about the environment. Furthermore, we establish hierarchy between various environment variables and model it as a TS. We demonstrate using case studies that this hierarchy allows the system to safely react in time to the events in the environment. \\ 
% % 4. We can deal with partial information. \\ 

% % }


==> IROS/literature.tex <==
% \vspace{3 pt}
\section{Related Works}\label{sec:literature}

% {\textcolor{brown}{
%     What exactly the symbolic representations capture?\\
%     Importance of symbolic planning methods for complex tasks with spatial and temporal modalities.\\
%     How do the existing methods address symbolic planning -  {\textit{symbolic planning and control for robot motion} \cite{belta2007symbolic} } - how do they handle perception inputs \\
%     some works to discuss : \\
%     1. Learning symbolic representations: {\textit{Constructing Abstraction Hierarchies Using a Skill-Symbol Loop \cite{konidaris2016constructing}, From Skills to Symbols: Learning Symbolic Representations 
% for Abstract High-Level Planning \cite{konidaris2018skills}}}
%     The hierarchical nature of human perception - a long-studied topic in psychology and human cognition}\\
%  }   
 
 
%  {\disharevised Literature review of reactive planning and hierarchical semantic representations and then the combinations of both}
 
%  \medskip
 
% \medskip

%
% \vspace{8pt}
{\disharevised 
% \subsection{Perception and Planning}
% \noindent{\textit{A. Perception and Planning: }}
%
%
% \textcolor{brown}{Story: perception-planning - one extreme is to have end-end learning \cite{pfeiffer2017perception} - not explainable, no gurantees on the robot behavior. On the other hand, we have modular approaches (for now we focus on perception) - in these approaches, knowledge is processed and utilized sequentially - while operating in complex and highly dynamic envs like SDC, these methods aim to have one-shot accurate detection - which is especially difficult to achieve in occluded envs. Building on top of these methods, some approaches consider obtaining high-level semantic information from the low-level sensor data before planning. This allows for 
% more complex tasks than simple point-to-point navigation, obstacle avoidance, etc., TL formalisms have been proven to be increasingly useful. 
% \cite{} - learning representation, etc.
% Some existing works address the problem of reactive planning by employing end-to-end learning frameworks. However, no guantees can be provided on the robot's behavior. 
% % \textit{In this work, we consider that the symbolic information is directly available and instead focus on its representation and reactive planning. This is a widely followed approach ~ \cite{kress2011mitigating}, etc.}
% There is limited literature on capturing different levels of detail in the environment - \cite{galindo2005multi} - anchoring, skill-sym loop, semantic SLAM, probabilistic semantic maps - direction for future research, etc. Specific to traffic signs, low and high features; Another line of research : perception-aware planning considers quantification of the incoming sensor information and favouring plans or policies that lead to more information - none of these approaches explicitly capture the relationships between symbols. 
% %
% % Our intuition is that reacting to varying levels of detail will result in safer reactions in face of edge cases. 
% Cite papers from psycho and then mention that our proposed representation is analogous to these. \cite{kantaros2022perception} - considers TL based planning with semantic SLAM in uncertain semantic envs - offline planning. 
% }
%
%Symbolic perception refers to a representation of the robot's perception information that captures its meaning and is amenable to formal methods. }
%
% The advent of data-driven approaches as well as rapid advances in image processing fields have greatly improved the low-level perception abilities (detection from direct sensor information) of autonomous cars~\cite{fridman2017autonomous,liang2020traffic, fayyad2020deep, tseng2018combination, laguna2014traffic}. On one hand, approaches such as \cite{https://doi.org/10.48550/arxiv.1604.07316} consider end-to-end learning producing real-time behavior however, these approaches often suffer from lack of explainability. On the other end of the spectrum lie modular approaches which break down the problem into a sequential perception-planning framework~\cite{okumura2016challenges, palmer1977hierarchical} and the references therein. These methods aim to have accurate real-time perception for efficient planning which is especially difficult to achieve in highly dynamic and complex environments. Building on top of these methods, some approaches consider obtaining high-level semantic information from the low-level sensor data before planning thus allowing for 
% more complex tasks than simple point-to-point navigation, obstacle avoidance, etc. 
%
% Our problem lies at the intersection of symbolic perception and reactive synthesis for temporal logic specifications. This section reviews the related works in these fields.
\smallskip
\iffalse
\noindent \textbf{\textit{Symbolic Perception: }}
% Our approach for the symbolic refinement tree representation is inspired by the way in which human brain processes varying levels of detail about the surroundings by utilizing highly-structured hierarchical data-structures enabling us to process complex situations e.g.,  \cite{palmer1977hierarchical, eckstein2020computational}, among others.
% . 
Our approach for symbolic refinement tree representation is inspired by the way in which human brain uses highly organized data-structures for abstracting varying levels of details in the surroundings to guide learning and decision-making e.g.,  \cite{palmer1977hierarchical, eckstein2020computational}.
% There is, however, limited literature on capturing and utilizing multiple levels of environment information in the context of robotics.
% \cite{galindo2005multi} address the problem of learning the ``anchoring" between the spatial and conceptual hierarchies for obtaining semantically similar regions in the environment. On the other hand, \cite{konidaris2016constructing} address the problem of learning abstract representations coupled with the agent's actions. As opposed to these approaches, where representation learning is the primary objective, we prescribe the symbolic representation that captures multiple levels of symbolic details from the environment. Learning these incremental symbolic relationships is a topic for future research. 
% \cite{galindo2005multi} address the problem of learning spatial and conceptual hierarchies in order to obtain semantically similar regions in the environment whereas \cite{konidaris2016constructing} explore learning abstract representations for perception coupled with agent's skills (actions). As opposed to these approaches, where representation learning is the primary objective, we prescribe the symbolic representation that captures multiple levels of symbolic details from the environment. Learning these incremental symbolic relationships is a topic for future research.  
With representation learning as the primary objective, \cite{galindo2005multi} propose learning hierarchies for obtaining semantically similar regions whereas \cite{konidaris2016constructing} explore learning abstract representations for perception coupled with agent's skills. On the other hand, our work prescribes symbolic representation and utilizes it for safe control synthesis; learning the symbolic relationships between the variables is a topic for future research. 
% \cite{galindo2005multi} presents a method for learning the ``anchoring" between the spatial and conceptual hierarchies for the given environment applied to mobile robots for obtaining semantically similar regions. On the other hand, \cite{konidaris2016constructing} address the problem of learning abstract representations coupled with the agent's actions. Here, higher levels of abstraction are learned as the agent acquires new skills (actions). In this work, we prescribe the symbolic representation that captures multiple levels of symbolic details from the environment. Learning these incremental symbolic relationships is a topic for future research. 

Some existing sensor fusion approaches for perception of autonomous vehicles consider varying levels of detection and processing of individual sensor information~\cite{fayyad2020deep}. Specific to traffic signs, \cite{fan2021multi}, \cite{liang2020traffic} propose the use of feature pyramids for neural networks that capture the low and high-level semantic information from a given image. Although the notion of capturing varying scales of features is a common thread, they address the problem of accurately detecting varying sized features from an image whereas, we capture the evolution with distance in symbolic knowledge about the environment.\\} 

% \smallskip
% % With respect to the perception for autonomous systems, numerous approaches ranging from learning-based techniques to SLAM have been proposed \cite{fayyad2020deep},~\cite{fridman2017autonomous},  \cite{tseng2018combination}, \cite{wang2018perception}. 
% Although the advent of data-driven approaches  as well as progress in image processing fields have greatly improved the  low-level perception abilities (detection from direct sensor information) of autonomous cars e.g.,~\cite{fridman2017autonomous,liang2020traffic, fayyad2020deep, tseng2018combination, laguna2014traffic}, the problems combining perception and decision-making are often dealt with in a sequential way \cite{okumura2016challenges}. That is the end-result obtained from the perception module is used as an input to the control synthesis module. %of autonomous systems
% Another line of research about perception and planning is extracting and leveraging the high-level symbolic information from the low-level sensor data e.g., using the semantic label \textit{``goal\_region}" from a set of pixels as an input. Many existing works deal with learning effective representations from given sensory data \cite{ghosh2018learning}, \cite{crespo2020semantic}. In this work, we assume that such a symbolic information is available to the system which is a widely followed approach for control synthesis \cite{kress2011mitigating}, \cite{kress-gazit_wheres_2007}, \cite{belta2007symbolic}, etc. 
% This is a widely followed approach for high-level control synthesis~\cite{belta2007symbolic}, \cite{kress2011mitigating}, \cite{kress2009temporal}, etc. 

% \vspace{-8pt}
% \textit{
% In this letter, we are interested in the symbolic information provided by the perception module. Thus, we abstract the way of collecting the information about the environment and instead consider that the symbolic information as an input to our planner. This is a widely followed approach for high-level control synthesis. }
% \textit{\textcolor{brown}{Even though this approach is widely-adopted, it may not result in an efficient reactive behavior under partial information TODO:\cite{}. As opposed to processing and extracting relevant representations from actual sensory data for perception (e.g., from vision and/or range sensors), we instead consider that such \textit{symbolic} representations of the environment information are provided. Many existing works deal with learning effective representations from given sensory data \cite{ghosh2018learning} \cite{crespo2020semantic}. 
%  }
% }
% \vspace{18 pt}
% %% Hierarchical representations
% \noindent\textcolor{blue}{
% % \subsection{Symbolic Representations}
% \textit{B. Symbolic Representations: }The use of symbolic information for robot planning and control \cite{belta2007symbolic}, \cite{kress2011mitigating}, \cite{kress2009temporal} has been considered before. However, these works
% do not consider leveraging the incremental perception knowledge and instead, assume full symbolic information for planning. The idea of capturing multiple levels of details in representations - though little explored in robotics in the context of information - has been long studied in cognitive psychology e.g., \cite{palmer1977hierarchical}. 
% The experiments presented in \cite{palmer1977hierarchical}, \cite{eckstein2020computational} indicate that human brain uses highly-structured and organized hierarchical data-structures to guide learning and decision-making where each level corresponds to varying levels of detail. }
% % The presented experiments indicate that the perceptual information in the human brain processes corresponds to a selectively organized data structures where each level corresponds to varying levels of detail. Furthermore, it was shown by \cite{eckstein2020computational} human brain uses hierarhical reinforcement learning approach which employs structure in the environment to guide learning and complex decision-making. 
% {\disharevised Within robotics, \cite{galindo2005multi} presents a method for learning the ``anchoring" between the spatial and conceptual hierarchies for the given environment applied to mobile robots for obtaining semantically similar regions. On the other hand, \cite{konidaris2016constructing} address the problem of learning abstract representations coupled with the agent's actions. Here, higher levels of abstraction are learned as the agent acquires new skills (actions). Specific to traffic signs, \cite{fan2021multi}, \cite{liang2020traffic} propose the use of feature pyramids for neural networks that capture the low and high-level semantic information. However, they are addressing a problem of accurately detecting varying sized features from the scene whereas, we are interested in capturing the evolution in symbolic information in knowledge about the environment. } 
% \vspace{5pt}\\
% some works consider hierarchical semantic representations. \cite{wang2018perception} where the hierarchy refers to the inter-relation between \textit{sense, plan, action} sequences,  TODO: read these:  \textit{Multimodal Hierarchical Dirichlet Process-Based Active Perception by a Robot, Multi-scale traffic sign detection model with attention, Multi-Hierarchical Semantic Maps for Mobile Robotics}. As opposed to these, our work focuses on utilizing the relationships that may exist in symbols obtained through possibly partial observations of the environment. To the authors' best knowledge, this is the first time that the multi-resolution symbolic representation of perception has been considered for reactive planning.
%
%
% reactive control

% \vspace{-4 mm}
% \subsection{Reactive Control Synthesis}
\noindent\textit{\textbf{{Temporal Logic-Based Reactive Control Synthesis:}}} {\disharevised Given the symbolic perception information and temporal logic goals,
\cite{vasile2020reactive} presents a sampling-based reactive planning approach  using potential functions to react to local request while ensuring infinite-time satisfaction of LTL tasks.} 
% \textcolor{brown}{\cite{saffiotti1997uses} - reviews fuzzy logic for autonomous navigation - even though fuzzy logic accounts for the numeric and symbolic aspects of reasoning, it doesnt allow to explicitly take into account the temporal aspects that are essential for specifying the rules of the road. 
\cite{8248668, brechtel2014probabilistic} describe decision making under perception uncertainty using approximate methods to solve the resulting partially observable Markov decision processes (POMDPs). On the contrary, we consider a wider, more complex set of rules and tasks while limiting the perception to a probabilistic setting.  % {\disharevised Temporal logics have been widely used to express complex mission specifications due to their rich expressivity. In this paper, our goal is to synthesize reactive control policies that satisfy the given specification not only for one but all possible behaviours of the environment. Generalized Reactivity (1), also referred to as assume-guarantee specifications are a subclass of Linear Temporal Logic (LTL) that can be synthesized in linear time as opposed to a general LTL formula that takes exponential time (in number of states -- double check!).} 


Assume-guarantee specifications reduce the otherwise computationally intensive, exponential-time synthesis problem as with LTL to a polynomial-time synthesis problem.
They have been used to obtain a verified reactive control plan for mobile robots in abstract dynamic environments \cite{kress2009temporal}. The authors propose a correct-by-construction hybrid reactive controller for bridging up the gap between low and high-level controllers.
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[scale=0.35, trim= 5cm 0cm 0cm 0cm]{IROS/images/motivation.png}
% % 	\vspace{-30pt}
% 	\caption{\small{A motivating example for leveraging partial knowledge about the environment for controlling the ego car. As the car does not have full view of the pedestrian sign, it may still slow down after recognizing the possibility of a warning sign and may have improved chances of reacting in time.}}
%  	\label{fig:motivation}
% 	\vspace{-15pt}
% \end{figure} 
% \indent Towards this end,
Within a similar context,
\cite{kress2011mitigating} solves a game between sensor propositions that represent the environment and robot propositions that represent the available control actions to synthesize a reactive control input. However, both of these works assume an accurate perception input.

{\disharevised Among the closely related works, \cite{fu2016optimal} consider probabilistic semantic maps provided by semantic SLAM algorithms and generate a control plan by converting a stochastic optimal control problem into a deterministic shortest path problem. On the other hand, \cite{kantaros2022perception} proposes a sampling-based multi-robot planning to generate reactive control policies based on semantic SLAM information given co-safe LTL specifications. Using Probabilistic Signal Temporal Logic specifications,
\cite{da2021active} proposes a counter-example-guided control synthesis, under perception uncertainty. In contrast to our approach, this approach requires accurate belief models of the perception that quantify the uncertainty of the perception system explicitly. None of the aforementioned works consider refinement in environment knowledge. As opposed to their approach for perception abstraction, in this work we consider a perception module wherein the information about the environment is incrementally improved and utilize the multi-resolution structure for safe control synthesis.}
\fi

 % the  abstraction of perception as a transition system whose transitions depend on the transitions in the control module. 
% {\color{red}[TODO: Double check]}. % checked it (sofie). 
 
% \indent  However, the map distributions considered in this work are fixed and so the candidate maps only depend on the confidence parameter. The approaches presented in \cite{kress2011mitigating}, \cite{wongpiromsarn_receding_2009}, \cite{filippidis2016control} consider assume-guarantee specifications for generating verified reactive plans. However, none of these works consider refinement in environment knowledge. As opposed to this, we address the problem of providing guarantees on system behavior for all valid environment behaviors while considering the incremental knowledge about environment states.}
% \indent With respect to the perception module of autonomous systems, numerous approaches have been proposed to improve the perception capabilities %of autonomous systems 
% ~\cite{fayyad2020deep},~\cite{fridman2017autonomous}, \cite{tseng2018combination}. Although the advent of data-driven approaches have greatly improved the perception abilities of autonomous cars, e.g.,~\cite{fridman2017autonomous}, the problems combining perception and decision-making are often dealt with in a sequential way. That is the end-result obtained from the perception module is used as an input to the control synthesis module \cite{okumura2016challenges}. 
%
%
% \indent These approaches do not consider the relationship that may exist in the learned symbols or parameters. For instance, consider an autonomous car going down the hill towards a pedestrian crossing as shown in Fig. \ref{TODO}. The blue rectangle represents the sensory range of the car. If the system waits for an exact output from the perception module, the car may have to travel further ahead until the sign fully comes into its sight. This may not leave enough time for the car to slow down to correctly take the pedestrian sign. However, if we consider the interactions between the perception and control modules based on the {\color{red} incremental ?} knowledge about the environment, the car may decide to slow down right after detecting a yellow board that there is possibly a ``warning sign" and may later on slow down further after detecting the sign completely. This underpins the need for considering multi-level interactions between perception and reactive control modules for the systems which may allow systems to react safely with the environment even when there is some degree of uncertainty associated with the learned parameters. 
%
% In this work, we propose a framework for high-level reactive control design given a symbolic perception input. Abstracting the way of collecting information about the environment state, we instead focus on leveraging the partial knowledge about these variables. The hierarchical relationships between learned variables aid in the decision making process for the ego car. The methods discussed in this work focus on the applications related to autonomous driving in urban environments. However, the proposed approach can be used in other settings wherein partial knowledge about the environment may lead to a safer control strategy. e.g., search-and-rescue tasks with priority. To achieve the verifiable usage of perception in motion planning and control as is present in autonomous driving, we will use abstractions to encapsulate the detection and estimation techniques. More precisely, combining the abstract models motion control and information gathering, we show that assume-guarantee specifications can be used to define and resolve traffic rules for cautious planning with perception.  
% % \noindent{\bfseries Approach.}
% % {\disha In this paper, we introduce a hierarchical perception framework for correct-by-construction reactive control synthesis.} To achieve the verifiable usage of machine learning in motion planning and control as is present in autonomous driving, we will use abstractions to encapsulate the learning algorithms. Furthermore, we will abstract the autonomous car into a finite model whose state action updates result both in atomic proposition, but we preserve the information captured by the cars behavior in the abstraction.  We show that this leads to an autonomous car that anticipates changes in traffic signs by slowing down and that actively checks the road condition while driving closer to a  light that can turn red at any moment. 
%  %
% %
% % More precisely, combining the abstract model of the machine learning algorithm and of the motion control and information gathering, we show that assume-guarantee specifications can be used to define and resolve traffic rules for cautious planning with perception and learning algorithms.
% %
% %% need for 
% The main contributions of this work are as follows: 1. We propose a framework for safe high-level reactive control with perception for an autonomous car. 2. We abstract the perception module and establish a hierarchy between these environment variables which facilitates the timely execution of necessary behavior that the system must perform in order to satisfy rules of the road. 3. Additionally, we demonstrate with the help of case studies that this hierarchy helps synthesizing control inputs even in case of partial information about the environment. 
%
% % We establish the inter-relation between the perception and control abstractions. 
%
% % {\disha Contributions: 1. The idea of establishing relations between various learned variables to make high-level decisions with safety guarantees.\\ 
% % 2. The inter-relation between evolution of the perception and control abstraction - The knowledge about the current state of the environment determines the behavior of the system which in the next step updates the knowledge about the environment and so on. \\ 
% % 3. We abstract the way of gathering information about the environment. Furthermore, we establish hierarchy between various environment variables and model it as a TS. We demonstrate using case studies that this hierarchy allows the system to safely react in time to the events in the environment. \\ 
% % 4. We can deal with partial information. \\ 
%
% % }


==> def.tex <==
%% Additional packages
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{cite}
%\usepackage{mathtools}
%\usepackage{calc}
%\usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{graphicx}
\usepackage{color}
\usepackage{url}
\usepackage{soul}
\usepackage[bookmarks=true]{hyperref}
%\usepackage{lineno}
%\usepackage{ulem} % for underlining and strike through
%\normalem % reset emph to normal
%\usepackage{setspace} % for line spacing - e.g. 1.5, 2
\usepackage[usenames,x11names]{xcolor}
\usepackage{xspace} % for inserting a space in TeX commands if needed
\usepackage{caption}
%\usepackage[numbers]{natbib}
\usepackage{multicol}
%\renewcommand{\thesubfigure}{\relax} % no subfig counters
%\let\chapter\section % algorithm2e natbib compatibility
%\usepackage{accents}
\usepackage[normalem]{ulem}

%% Packages
%\usepackage[margin=1in]{geometry}
%\usepackage[abs]{overpic}
\usepackage[linesnumbered,vlined,ruled]{algorithm2e}
\usepackage{multirow} % for cell tables spanning multiple rows
\usepackage{tikz,pgf}
% \usetikzlibrary{arrows,automata,shapes,calc,backgrounds,spy,positioning,shadows}
%\usetikzlibrary{external}
%\tikzexternalize
%\usepackage[sort,round]{natbib}
%\usepackage{lipsum}

%\usepackage[author={Cristi}]{pdfcomment}

%%% figure path
\graphicspath{{figures/}}

%% Remove footnote mark
%\renewcommand{\footnotemark}{}

%%% Redefine qed symbol
%\renewcommand{\qedsymbol}{$\blacksquare$}

%% Projection symbol
%\newcommand{\project}[1]{\! \upharpoonright_{#1}}

\SetKw{Break}{break}

%% Theorems 
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{example}{Example}[section]
\newtheorem{algo}{Algorithm}
\newtheorem{problem}{Problem}[section]
\newtheorem{Procedure}[theorem]{Procedure}
\newtheorem{assumption}{Assumption}
\newcommand{\exampler}[2]{\medskip \hskip -\parindent {\bf Example #1 Revisited.~}{\it #2}\medskip}

%% Percent
%\newcommand\oprocendsymbol{\hbox{$\square$}}
%\newcommand\oprocend{\relax\ifmmode\else\unskip\hfill\fi\oprocendsymbol}
%\def\eqoprocend{\tag*{$\bullet$}}

%% Enumerate environment
%\renewcommand{\labelenumi}{(\roman{enumi})}
%\renewcommand{\labelenumii}{(\alph{enumii})}

%% Breakable comma
%\mathchardef\breakingcomma\mathcode`\,
%{\catcode`,=\active
%  \gdef,{\breakingcomma\discretionary{}{}{}}
%}
%\newcommand{\breqn}[1]{\mathcode`\,=\string"8000 #1}

%% Other Stuff
\newcommand{\margin}[1]{\marginpar{\tiny\color{blue} #1}}
%%\addtolength{\marginparwidth}{-0.3in}
\newcommand{\todo}[1]{\vskip 0.05in \colorbox{yellow}{$\Box$ \ttfamily\bfseries\small#1}\vskip 0.05in}
%\newcommand{\todo}[1]{}
%\newcommand{\vers}{\operatorname{vers}}
% \highlight[<colour>]{<stuff>}
\newcommand{\highlight}[2][yellow]{\mathchoice%
  {\colorbox{#1}{$\displaystyle#2$}}%
  {\colorbox{#1}{$\textstyle#2$}}%
  {\colorbox{#1}{$\scriptstyle#2$}}%
  {\colorbox{#1}{$\scriptscriptstyle#2$}}}%

\newcommand{\disha}{\color{black}}

\newcommand{\dishalatest}{\color{cyan}}
\newcommand{\dishanew}{\color{black}}
\renewcommand\baselinestretch{0.98}\selectfont
% \setlength{\bibsep}{0ex}
%% Roman, calligraphic, boldface, double barred letters
\newcommand{\RM}[1]{\mathrm{#1}}
\newcommand{\CA}[1]{\mathcal{#1}}
\newcommand{\BF}[1]{\mathbf{#1}}
\newcommand{\BB}[1]{\mathbb{#1}}
\newcommand{\TT}[1]{\mathtt{#1}}
\newcommand{\BS}[1]{\boldsymbol{#1}}

%% Temporal logic symbols
% \newcommand{\Next}{\BF{X}}
% \newcommand{\Always}{\BF{G}}
% \newcommand{\Event}{\BF{F}}
% \newcommand{\Until}{\CA{U}}
% \newcommand{\Implies}{\Rightarrow}
\newcommand{\True}{\top}
\newcommand{\False}{\perp}
\newcommand{\trap}{\bowtie}
\newcommand{\virtual}{\rhd}

\newcommand{\AP}{{AP}}
\newcommand{\Pref}{{R}}

%% Abbreviations
%\def\eg{e.g.\xspace}
%\def\Eg{E.g.\xspace}
%\def\ie{i.e.\xspace}
%\def\Ie{I.e.\xspace}
%\def\etc{etc.\xspace}
%\def\vs{vs.\xspace}
%\def\wrt{w.r.t.\xspace}
%\def\etal{et al.\xspace}

%% Exotic words
\newcommand{\buchi}{B\"uchi\ }

%% Symbols of automata
\newcommand{\PA}{\mathcal{P}}
\newcommand{\BA}{\mathcal{B}}
%\newcommand{\FA}{\mathcal{F}}
\newcommand{\FA}{\mathcal{A}}
\newcommand{\TS}{\mathcal{T}}
\newcommand{\LA}{\mathcal{L}}
\newcommand{\KA}{\mathcal{K}}
\newcommand{\ES}{\mathcal{E}}

%% Short macros for arrows
\newcommand{\ras}[1]{\stackrel{#1}{\to}}
% \newcommand{\rasp}[2]{\overset{#1}{\underset{#2}{\to}}}
\newcommand{\rasp}[2]{\overset{#1\mid #2}{\to}}

%% Names of the Algorithms
%\newcommand{\optrun}{\textsc{Optimal-Run}\ }
%\newcommand{\exactmultioptrun}{\textsc{Exact-Multi-Robot-Optimal-Run}\ }
%\newcommand{\constR}{\textsc{Construct-Region-Automaton}\ }
%\newcommand{\constT}{\textsc{Construct-Team-TS}\ }
%\newcommand{\syncT}{\textsc{Sync-Team-TS}\ }
%\newcommand{\boundOpt}{\textsc{Bound-Optimality}\ }

% Custom operators
%\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\norm}[1]{\left\| {#1} \right\|}
\newcommand{\normu}[1]{\left\| {#1} \right\|_{U}}
\newcommand{\norml}[1]{\left\| {#1} \right\|_{L}}
\newcommand{\norminf}[1]{\left\| {#1} \right\|_{\infty}}
\newcommand{\normeucl}[1]{\left\| {#1} \right\|_{2}}
\newcommand{\abs}[1]{\left| {#1} \right|}
\newcommand{\card}[1]{\left| {#1} \right|}
\newcommand{\spow}[1]{2^{#1}}
% \newcommand{\trel}[1]{\left| {#1} \right|_{TR}}
% \newcommand{\btrel}[1]{\left| {#1} \right|_{BTR}}
% \newcommand{\ltrel}[1]{\left| {#1} \right|_{LTR}}
\newcommand{\lrel}[1]{\left| {#1} \right|_{LR}}
\newcommand{\indicator}{\chi}
%\newcommand{\interior}[1]{\accentset{\smash{\raisebox{-0.12ex}{$\scriptstyle\circ$}}}{#1}\rule{0pt}{2.3ex}}
\newcommand{\interior}[1]{\mathring{#1}}
\newcommand{\prefix}[1]{P\left({#1}\right)}
\newcommand{\dto}{\rightrightarrows}
\newcommand{\range}[1]{\left[\left[{#1}\right]\right]}
\newcommand{\any}{\bullet}
\newcommand{\R}{\mathbb{R}}
\newcommand{\TS}{\mathcal{T}}
%
%% Display a grid to help align images
%\beamertemplategridbackground[1cm]


